Spectropolarimetry of SN 2023ixf reveals both circumstellar material and helium core to be aspherical

We present multi-epoch optical spectropolarimetric and imaging polarimetric observations of the nearby Type II supernova (SN) 2023ixf discovered in M101 at a distance of 6.85 Mpc. The first imaging polarimetric observations were taken +2.33 days (60085.08 MJD) after the explosion, while the last imaging polarimetric data points (+73.19 and +76.19 days) were acquired after the fall from the light curve plateau. At +2.33 days there is strong evidence of circumstellar material (CSM) interaction in the spectra and the light curve. A significant level of intrinsic polarization $p_r = 1.02\pm 0.07 \% $ is seen during this phase which indicates that this CSM is aspherical. We find that the polarization evolves with time toward the interstellar polarization level during the photospheric phase, which suggests that the recombination photosphere is spherically symmetric. There is a jump in polarization ($p_r =0.45 \pm 0.08 \% $ and $p_r =0.62 \pm 0.08 \% $) at +73.19 and +76.19 days when the light curve falls from the plateau. This is a phase where polarimetric data is sensitive to non-spherical inner ejecta or a decrease in optical depth into the single scattering regime. We also present spectropolarimetric data that reveal line (de)polarization during most of the observed epochs. In addition, at +14.50 days we see an ``inverse P Cygni" profile in the H and He line polarization, which clearly indicates the presence of asymmetrically distributed material overlying the photosphere. The overall temporal evolution of polarization is typical for Type II SNe, but the high level of polarization during the rising phase has only been observed in SN 2023ixf.

==> author.tex <==
\author[0000-0002-4022-1874]{Manisha Shrestha}
\UA


\author[0000-0002-3452-0560]{G. Grant Williams}
\MMT
\UA

\author[0000-0002-3452-0560]{Sabrin DeSoto}
\DU



\author[0000-0003-4102-380X]{David J. Sand}
\UA

\author[0000-0002-0744-0047]{Jeniveve Pearson}
\UA


\author[0000-0002-0832-2974]{Griffin Hosseinzadeh}
\UA

\author[0000-0002-4924-444X]{K. Azalee Bostroem}
\catalyst\UA


\author[0000-0003-0123-0062]{Jennifer E. Andrews}
\GeminiNorth

\author[0000-0002-7937-6371]{Yize Dong \begin{CJK*}{UTF8}{gbsn}(董一泽)\end{CJK*}}
\UCD



\author[0000-0003-2744-4755]{Emily Hoang}
\UCD

\author[0000-0003-0549-3281]{Daryl Janzen}
\USask
\author[0000-0001-5754-4007]{Jacob E. Jencson}
\IPACMR

\author[0000-0001-9589-3793]{M.~J. Lundquist}

\Keck
\author{Darshana Mehta}
\UCD

\author[0000-0002-7015-3446]{Nicol\'as Meza Retamal}
\UCD

\author[0000-0001-8818-0795]{Stefano Valenti}
\UCD

\author[0000-0002-8826-3571]{Christopher Bilinski}
\UA

\author[0000-0003-1495-227]{Jennifer L. Hoffman}
\DU

\author[0000-0002-5083-3663]{Paul S. Smith}
\UA
\author[]{Peter Milne}
\UA

\author[]{Doug Leonard}
\SDS



\author{Phil Daly}
\UA



\author[0000-0003-4253-656X]{D.\ Andrew Howell}
\LCO\UCSB
\author[0000-0001-5807-7893]{Curtis McCully}
\LCO
\UCSB

\author[0000-0003-0209-9246]{Estefania Padilla Gonzalez}
\LCO
\UCSB
\author[0000-0002-7472-1279]{Craig Pellegrino}
\LCO 
\UCSB
\author[0000-0003-0794-5982]{Giacomo Terreran}
\LCO 
\UCSB



\author{Megan Newsome}
\LCO 
\UCSB

\author{Joseph Farah}
\LCO 
\UCSB


\author[0000-0001-5510-2424]{Nathan Smith}
\UA

\









